Streaming of rendered content with adaptive frame rate and resolution

Streaming rendered content is an attractive way to bring high-quality graphics to billions of mobile devices that do not have sufficient rendering power. Existing solutions render content on a server at a fixed frame rate, typically 30 or 60 frames per second, and reduce resolution when bandwidth is restricted. However, this strategy leads to suboptimal rendering quality under the bandwidth constraints. In this work, we exploit the spatio-temporal limits of the human visual system to improve perceived quality while reducing rendering costs by adaptively adjusting both frame rate and resolution based on scene content and motion. Our approach is codec-agnostic and requires only minimal modifications to existing rendering infrastructure. We propose a system in which a lightweight neural network predicts the optimal combination of frame rate and resolution for a given transmission bandwidth, content, and motion velocity. This prediction significantly enhances perceptual quality while minimizing computational cost under bandwidth constraints. The network is trained on a large dataset of rendered content labeled with a perceptual video quality metric. The dataset and further information can be found at the project web page: https://www.cl.cam.ac.uk/research/rainbow/projects/adaptive_streaming/.

==> custom_commands.tex <==
\RequirePackage{letltxmacro}
\RequirePackage{xspace}
\RequirePackage{nicefrac}

\newcommand{\cdms}{\,cd/m$^2$\xspace}
\newcommand{\degpers}{\,\nicefrac{deg}{s}\xspace}

\newcommand{\cond}[1]{{\fontfamily{cmss}\selectfont{#1}}}

\newcommand{\JM}[1]{\textcolor{red!70!black}{\textnormal{(Joe) #1}}}

\newcommand{\YL}[1]{\textcolor{green!60!black}{\textnormal{(Yaru) #1}}}
% \newcommand{\todo}[1]{\textcolor{red}{\textnormal{\textbf{todo:} #1}}}
\newcommand{\todo}[1]{\textcolor{red}{\textnormal{\textnormal{} #1}}}

\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{algo:#1}}
\newcommand{\chapterref}[1]{Chapter~\ref{chapter:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tableref}[1]{Table~\ref{tab:#1}}
\newcommand{\etal}{et al.\xspace}
%\newcommand{\degpers}{\,\nicefrac{deg}{s}\xspace}
\newcommand{\degperssq}{\,\nicefrac{deg}{s\textsuperscript{2}}\xspace}
\newcommand{\degree}{$^{\circ}$\xspace}
\newcommand{\Hz}{\,Hz\xspace}
\newcommand{\fourier}{\mathfrak{F}}
\newcommand{\infourier}{^{\mathfrak{F}}}

\LetLtxMacro{\originaleqref}{\eqref}
\renewcommand{\eqref}[1]{Eq.~\originaleqref{eq:#1}}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

% \newcommand{\todo}[1]{\textcolor{red}{\textbf{todo: #1}}}
\newcommand{\RM}[1]{\textcolor{brown}{\textnormal{(Rafal) #1}}}

\newcommand{\ourmethod}{Name-of-your-method}

\newcommand{\code}[1]{\texttt{#1}}

\newcommand{\supplementary}{Supplementary}

% Use for subscript/index that is NOT a variable (index)
\newcommand{\ind}[1]{\text{#1}}


% Use this macro to mark your changes in the revision
\newcommand{\newedit}[1]{\textcolor{red}{\textnormal{\textbf{NEWEDIT:} #1}}}
\newcommand{\edit}[1]{\textcolor{black}{{#1}}}
%____________________________________________________________________________________________


